Transfer learning for time series classification using synthetic data generation

In this paper, we propose an innovative Transfer learning for Time series classification method. Instead of using an existing dataset from the UCR archive as the source dataset, we generated a 15,000,000 synthetic univariate time series dataset that was created using our unique synthetic time series generator algorithm which can generate data with diverse patterns and angles and different sequence lengths. Furthermore, instead of using classification tasks provided by the UCR archive as the source task as previous studies did,we used our own 55 regression tasks as the source tasks, which produced better results than selecting classification tasks from the UCR archive

==> cover.tex <==
\begin{center}
    \vspace*{1cm}
    
   
    
    \vspace{2cm}
    
    {\Large \textbf{Transfer learning for time series classification using synthetic data generation}}
    
    \vspace{1.5cm}
    
    Yarden Rotem ,\qquad  Nathaniel Shimoni,\qquad Lior Rokach,\qquad Bracha Shapira \\
    \textit{Software and Information Systems Engineering} \\
    \textit{Ben-Gurion University of the Negev}\\
    Be'er Sheva, Israel \\
    Email: \{rotemyar, nathanie, liorrk, bshapira\}@post.bgu.ac.il

    
    \vspace{1cm}
    
    In this paper, we propose an innovative Transfer learning for Time series classification method. Instead of using an existing dataset from the UCR archive as the source dataset, we generated a 15,000,000 synthetic univariate time series dataset that was created using our unique synthetic time series generator algorithm which can generate data with diverse patterns and angles and different sequence lengths. Furthermore, instead of using classification tasks provided by the UCR archive as the source task as previous studies did,we used our own 55 regression tasks as the source tasks, which produced better results than selecting classification tasks from the UCR archive.
    
    
  \vfill
    

\end{center}
